Skill over Scale: The Case for Medium, Domain-Specific Models for SE

Recent advancements in AI have sparked a trend in constructing large, generalist language models that handle a multitude of tasks, including many code-related ones. While these models are expensive to train and are often closed-source, they have enjoyed broad adoption because they tend to outperform smaller, domain-specific models of code. In this work, we argue that this is not a foregone conclusion. We show that modestly sized domain-specific models can outperform much larger ones on code labeling tasks, provided they are trained to the same standards. Concretely, we focus on StackOverflow (SO), which offers large volumes of aligned code and text data. We align established best-practices for pre-training large language models with properties of SO as a data source, especially using a large context window (2,048 tokens), coupled with a powerful toolkit (Megatron-LM) to train two models: SOBertBase (125M parameters) and SOBertLarge (762M parameters), at a budget of just $374 and $1600 each. We compare the performance of our models with a prior domain-specific model which did not adopt many of these practices (BERTOverflow), as well two general-purpose BERT models and two models in OpenAI's GPT series (GPT-3.5 and GPT-4). We study four labeling tasks: question quality prediction, closed question prediction, NER and obsoletion prediction. The final task is a new benchmark we introduce, on which we additionally compare SOBert with a fine-tuned CodeLlama and StackLlama (models with 10x more parameters than SOBertLarge). Our models consistently outperform all baselines. In contrast, BertOverflow is outperformed by generalist models in most tasks. These results demonstrate that pre-training both extensively and properly on in-domain data can yield a powerful and affordable alternative to leveraging closed-source general-purpose models. Both models are released to the public on Hugging Face.

==> sections/Threat.tex <==
% \added{In this section, we will discuss potential threats to the validity of our study, acknowledging limitations and factors that might affect the interpretation of our findings.

% \textbf{Quality-Based Focus:} Focusing on posts with indicators of quality allows us to better evaluate model performance on content likely to be useful in practice. However, we acknowledge this filtering process means our models may not perform as well on lower quality posts. An interesting area for future work would be to analyze model performance on the full distribution of post quality and community engagement. We could also experiment with different filtering thresholds like 2+ upvotes. Overall, we aimed to balance gathering a sufficient volume of quality data versus maximizing coverage of the entire corpus.

% \textbf{Scope of Model Comparisons:} In this study, we focused our experiments on comparing SOBert against BERT models trained on a general corpus as well as the StackOverflow-specific BERTOverflow. However, we acknowledge that other relevant models have been proposed for learning representations of StackOverflow data, such as seBERT, PTM4Tag and Post2Vec. We did not include comparisons against these other StackOverflow-specific models due to differences in model architecture, training data, and intended applications. 

% For example, seBERT incorporates additional data sources beyond StackOverflow during pre-training, PTM4Tag specifically models the Title, Description and Code components of StackOverflow questions which differing from our broader objective of modelling StackOverflow answers and their corresponding comments to capture the temporal evolution of information within the answers. We didn't include Post2Vec in our baseline as Post2Vec exhibited inferior performance in the Tag recommendation downstream task in comparison to PTM4Tag.


% While comparing against these related models would lend further insights, we leave this analysis to future work and focused our experiments on validating SOBert against generic BERT models and the most similar StackOverflow-specific baseline in BERTOverflow. More extensive comparisons assessing relative strengths and weaknesses of the growing number of StackOverflow language models remains an interesting area for further research.

% \textbf{Limitations in GPT-3.5 Comparisons:} In our comparisons with ChatGPT, we were only able to evaluate its performance using 0-shot and 3-shot prompting due to constraints imposed by the API. This limited the variety of prompts we could test, which could impact the completeness of our analysis. However, zero-shot and three-shot prompting represent reasonable baseline settings for evaluating few-shot learning capabilities. The substantially lower accuracy of ChatGPT even with three examples suggests that purely few-shot prompting is unlikely to compensate for its lack of task-specific fine-tuning. While more comprehensive prompting strategies could lend additional insights, the sizable gaps between ChatGPT and SOBert under standard prompting provide meaningful evidence that task-specific training remains critical for strong performance on downstream tasks, even for large language models. The prompting constraints do not undermine the validity of our core findings regarding the value of specialized pre-training.

% \textbf{Exclusion of GPT-4:} We did not include comparisons with GPT-4 in our study due to its unavailability during our experiments. This decision may have implications for the scope of our findings.}



















% % In this study, we undertook a deliberate approach to enhance the quality and relevance of our experiments by focusing on posts with indicators of quality. By doing so, we aimed to better evaluate the performance of our SOBert model on content that is likely to be useful in practical Software Engineering (SE) related applications. However, it is essential to acknowledge that this filtering process may introduce potential threats to the validity of our findings. Specifically, our models may not perform as effectively on lower quality posts or those with limited community engagement.

% % An interesting avenue for future research would be to analyze the performance of our models on the full distribution of post quality and community engagement. Additionally, experimenting with different filtering thresholds, such as including posts with 2 or more upvotes, could provide valuable insights. Striking the right balance between gathering a sufficient volume of quality data and maximizing coverage of the entire corpus is a challenge that warrants further investigation.

% % Another aspect that warrants consideration is the scope of our model comparisons. We chose to focus our experiments on contrasting SOBert with general BERT models and the StackOverflow-specific BERTOverflow. However, it is essential to recognize that other relevant models have been proposed for learning representations of StackOverflow data, including seBERT \cite{von2021validity}, Post2Vec \cite{xu2021post2vec}, and PTM4Tag\cite{he2022ptm4tag}.

% % We did not include comparisons against these other StackOverflow-specific models in our study due to substantial differences in model architecture, training data, and intended applications. For instance, seBERT \cite{von2021validity} incorporates additional data sources beyond StackOverflow during pretraining, while Post2Vec \cite{xu2021post2vec} is primarily designed for post representation learning rather than downstream task performance. PTM4Tag\cite{he2022ptm4tag}, on the other hand, is tailored specifically for tag prediction, which differs from our broader range of tasks.

% % While comparing SOBert against these related models could provide further insights into its strengths and weaknesses, we have chosen to leave this analysis to future work. Our primary focus was on validating SOBert against generic BERT models and the most similar StackOverflow-specific baseline, BERTOverflow \cite{tabassum2020code}. 

% % Additionally, it is worth noting that we did not compare SOBert with GPT-4 in this study. This decision was based on various factors, including the unavailability of GPT-4 during the time of our experiments, differences in model architectures, and the focus of our research on the StackOverflow domain. GPT-4 may introduce unique capabilities and characteristics that could influence the comparative results.

% \added{ We evaluated the performance of various pre-trained models using implementations provided by the popular open-source community HuggingFace \footnote{https://huggingface.co/jeniya/BERTOverflow}\footnote{https://huggingface.co/bert-base-uncased}\footnote{https://huggingface.co/bert-large-uncased} and are thus dependent on their quality of model implementations. 
% \added{While our assessment of SOBert includes a comprehensive analysis of four downstream tasks from well-established sources, it is important to recognize that the applicability of our findings to different tasks may differ. 

% We did not include comparisons with GPT-4 in our study due to its unavailability during our experiments. Additionally, the nature of API access from OpenAI implies that the performance of the language model can fluctuate over time due to model updates without prior notification, potentially affecting its performance. We were also restricted by API limitations for the number of samples we could prompt for and the number of examples provided in the prompt. However, the fact that the LLM is much less accurate in each task implies that it is unlikely to be able to bridge the absence of task specific training with examples alone.}

==> tables.tex <==
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|lllll|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Model}} &
%   \multicolumn{1}{l|}{\textbf{Weighted accuracy}} &
%   \multicolumn{1}{l|}{\textbf{Weighted precision}} &
%   \multicolumn{1}{l|}{\textbf{Weighted Recall}} &
%   \textbf{F1 Score} \\ \hline
% \multicolumn{5}{|l|}{\textbf{Test Set}} \\ \hline
% \multicolumn{1}{|l|}{BertOverflow} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.6877} &
%   \multicolumn{1}{l|}{0.6747} &
%   0.6812 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{BBUBase}} &
%   \multicolumn{1}{l|}{\multirow{2}{*}{}} &
%   \multicolumn{1}{l|}{0.815} &
%   \multicolumn{1}{l|}{0.564} &
%   0.624 \\ \cline{3-5} 
% \multicolumn{1}{|l|}{} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.7702} &
%   \multicolumn{1}{l|}{0.4592} &
%   0.5754 \\ \hline
% \multicolumn{1}{|l|}{BBULarge} &
%   \multicolumn{1}{l|}{0.563} &
%   \multicolumn{1}{l|}{0.826} &
%   \multicolumn{1}{l|}{0.563} &
%   0.625 \\ \hline
% \multicolumn{1}{|l|}{\textbf{SOBertBase}} &
%   \multicolumn{1}{l|}{\textbf{0.773}} &
%   \multicolumn{1}{l|}{\textbf{0.896}} &
%   \multicolumn{1}{l|}{\textbf{0.773}} &
%   \textbf{0.819} \\ \hline
% \multicolumn{1}{|l|}{\textbf{SOBertLarge}} &
%   \multicolumn{1}{l|}{\textbf{0.769}} &
%   \multicolumn{1}{l|}{\textbf{0.891}} &
%   \multicolumn{1}{l|}{\textbf{0.769}} &
%   \textbf{0.815} \\ \hline
% \multicolumn{1}{|l|}{SoftNER} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.7842} &
%   \multicolumn{1}{l|}{0.7979} &
%   0.7910 \\ \hline
% \multicolumn{5}{|l|}{\textbf{Dev Set}} \\ \hline
% \multicolumn{1}{|l|}{BertOverflow} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.7211} &
%   \multicolumn{1}{l|}{0.7051} &
%   0.7130 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{BBUBase}} &
%   \multicolumn{1}{l|}{\multirow{2}{*}{}} &
%   \multicolumn{1}{l|}{0.83} &
%   \multicolumn{1}{l|}{0.573} &
%   0.634 \\ \cline{3-5} 
% \multicolumn{1}{|l|}{} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.7957} &
%   \multicolumn{1}{l|}{0.4642} &
%   0.5864 \\ \hline
% \multicolumn{1}{|l|}{BBULarge} &
%   \multicolumn{1}{l|}{0.57} &
%   \multicolumn{1}{l|}{0.836} &
%   \multicolumn{1}{l|}{0.57} &
%   0.632 \\ \hline
% \multicolumn{1}{|l|}{\textbf{SOBertBase}} &
%   \multicolumn{1}{l|}{\textbf{0.775}} &
%   \multicolumn{1}{l|}{\textbf{0.903}} &
%   \multicolumn{1}{l|}{\textbf{0.775}} &
%   \textbf{0.823} \\ \hline
% \multicolumn{1}{|l|}{\textbf{SOBertLarge}} &
%   \multicolumn{1}{l|}{\textbf{0.779}} &
%   \multicolumn{1}{l|}{\textbf{0.904}} &
%   \multicolumn{1}{l|}{\textbf{0.779}} &
%   \textbf{0.826} \\ \hline
% \multicolumn{1}{|l|}{SoftNER} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.7881} &
%   \multicolumn{1}{l|}{0.8172} &
%   0.8024 \\ \hline
% \end{tabular}%
% }
% \caption{Evaluation on the dev and test sets of the StackOverflow NER corpus. SOBert outperforms the existing approaches.}
% \label{tab:NER}
% \end{table}







% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% Model               & Hyperparam BS, LR, max Seq Length & Weighted accuracy & Weighted precision & Weighted Recall & F1 Score      \\ \hline
% BertOverflow        & 32,1e-5,512                       & 0.72              & 0.72               & 0.72            & 0.72          \\ \hline
% BBUBase             & 32,1e-5,512                       & 0.82              & 0.83               & 0.82            & 0.82          \\ \hline
% BBULarge            & 32,1e-5,512                       & 0.71              & 0.72               & 0.71            & 0.71          \\ \hline
% \textbf{SOBertBase} & \textbf{32,1e-5,512}              & \textbf{0.86}     & \textbf{0.86}      & \textbf{0.86}   & \textbf{0.86} \\ \hline
% \textbf{SOBertLarge} &
%   \textbf{\begin{tabular}[c]{@{}l@{}}16,1e-5,512\\ (gradient accumulation=2)\end{tabular}} &
%   \textbf{0.91} &
%   \textbf{0.91} &
%   \textbf{0.91} &
%   \textbf{0.91} \\ \hline
% \end{tabular}%
% }
% \caption{Evaluation on the StackOverflow Quality Tag prediction dataset. SOBert outperforms the existing approaches.}
% \label{tab:Tag}
% \end{table}







\begin{table}[!ht]


\begin{tabular}{p{2cm} p{1.4cm} p{1cm} p{1cm} p{0.5cm} p{0.5cm}}
\toprule
\textbf{Task} & \textbf{Model} & \textbf{Balanced Accuracy} & \textbf{Weighted Precision} & \textbf{Recall} & \textbf{F1-Score} \\
\midrule
\multirow{5}{*}{\includegraphics[height=1.5em]{sections/Images/3.png} NER} & BertOverflow & -- & 0.69 & 0.67 & 0.68
 \\
& BBUBase & -- & 0.80 & 0.46 & 0.55 \\
& BBULarge & 0.56 & 0.83 & 0.56 & 0.63
\\
& SOBertBase & \textbf{0.88} & \textbf{0.93} & 0.88 & \textbf{0.90} \\
& SOBertLarge & 0.83 & 0.86&\textbf{0.93}&0.83\\
& SoftNER & -- & 0.78 & 0.80 & 0.79
\\
\midrule
\multirow{5}{*}{\includegraphics[height=1.5em]{sections/Images/1.png} Quality} & BertOverflow & 0.72 & 0.72 & 0.72 & 0.72 \\
& BBUBase & 0.82 & 0.83 & 0.82 & 0.82 \\
& BBULarge & 0.71 & 0.72 & 0.71 & 0.71 \\
& SOBertBase & 0.86 & 0.86 & 0.86 & 0.86 \\
& SOBertLarge &\textbf{0.92} & \textbf{0.92} & \textbf{0.92} & \textbf{0.92} \\
\midrule
\multirow{5}{*}{\includegraphics[height=1.5em]{sections/Images/2.png} Closed Question} & BertOverflow & 0.53 & 0.49 & 0.53 & 0.41 \\
& BBUBase & 0.60 & 0.56 & 0.60 & 0.56 \\
& BBULarge & 0.53 & 0.48 & 0.53 & 0.43 \\
& SOBertBase & \textbf{0.63 }& \textbf{0.62 }& \textbf{0.63 }& \textbf{0.61} \\
& SOBertLarge & \textbf{0.63} & 0.61 & \textbf{0.63} & \textbf{0.61} \\
\midrule
\multirow{5}{*}{\includegraphics[height=1.5em]{sections/Images/4.png} Obsoletion} & BertOverflow & 0.49 & 0.47 & 0.49 & 0.48 \\
& BBUBase & 0.70 & 0.70 & 0.70 & 0.70 \\
& BBULarge & 0.48 & 0.47 & 0.48 & 0.47 \\
& SOBertBase & \textbf{0.92} & {0.76} & \textbf{0.92} & \textbf{0.82} \\
& SOBertLarge & {0.71} & \textbf{0.81} & {0.71} & {0.75} \\
\bottomrule
\end{tabular}
\caption{Performance Metrics for the Models Across the 4 Tasks - Named Entity Recognition (NER), Quality Prediction, Closed Question Prediction, and Obsoletion Detection }
\label{tab:results}
\end{table}



